Towards Fair and Efficient Learning-based Congestion Control

Recent years have witnessed a plethora of learning-based solutions for congestion control (CC) that demonstrate better performance over traditional TCP schemes. However, they fail to provide consistently good convergence properties, including {\em fairness}, {\em fast convergence} and {\em stability}, due to the mismatch between their objective functions and these properties. Despite being intuitive, integrating these properties into existing learning-based CC is challenging, because: 1) their training environments are designed for the performance optimization of single flow but incapable of cooperative multi-flow optimization, and 2) there is no directly measurable metric to represent these properties into the training objective function. We present Astraea, a new learning-based congestion control that ensures fast convergence to fairness with stability. At the heart of Astraea is a multi-agent deep reinforcement learning framework that explicitly optimizes these convergence properties during the training process by enabling the learning of interactive policy between multiple competing flows, while maintaining high performance. We further build a faithful multi-flow environment that emulates the competing behaviors of concurrent flows, explicitly expressing convergence properties to enable their optimization during training. We have fully implemented Astraea and our comprehensive experiments show that Astraea can quickly converge to fairness point and exhibit better stability than its counterparts. For example, \sys achieves near-optimal bandwidth sharing (i.e., fairness) when multiple flows compete for the same bottleneck, delivers up to 8.4$\times$ faster convergence speed and 2.8$\times$ smaller throughput deviation, while achieving comparable or even better performance over prior solutions.

==> Makefile <==
DOCUMENT=main

default: $(DOCUMENT).pdf

$(DOCUMENT).toc: $(DOCUMENT).tex
	pdflatex $(DOCUMENT).tex

$(DOCUMENT).pdf: $(DOCUMENT).toc
	bibtex $(DOCUMENT)
	pdflatex $(DOCUMENT).tex
	pdflatex $(DOCUMENT).tex

#--------------------------------------------------
# $(DOCUMENT).ps: $(DOCUMENT).dvi
# 	dvips -t letter -Ppdf -G0 -o $@ $<
# 
# $(DOCUMENT).pdf: $(DOCUMENT).ps
# 	cat $(DOCUMENT).ps | ps2pdf - > $(DOCUMENT).pdf 
#-------------------------------------------------- 

all: $(DOCUMENT).pdf

clean:
	rm -rf *.aux $(DOCUMENT).log $(DOCUMENT).toc \
     $(DOCUMENT).bbl $(DOCUMENT).blg $(DOCUMENT).pdf $(DOCUMENT).out \


==> macros.tex <==


% Make the section headings smaller.
\usepackage[small, compact]{titlesec}
\titlespacing*{\section}{0pt}{3pt}{2pt}
\titlespacing*{\subsection}{0pt}{2pt}{2pt}
\titlespacing*{\subsubsection}{0pt}{2pt}{2pt}

% Do not penalize widow and orphan lines
\widowpenalty=0 % Allow the end of a paragraph to overflow to the next page
\clubpenalty=0  % Allow the beginning of a paragraph to begin from the prev page
\brokenpenalty=0

\def\UrlBreaks{\do\A\do\B\do\C\do\D\do\E\do\F\do\G\do\H\do\I\do\J
	\do\K\do\L\do\M\do\N\do\O\do\P\do\Q\do\R\do\S\do\T\do\U\do\V
	\do\W\do\X\do\Y\do\Z\do\[\do\\\do\]\do\^\do\_\do\`\do\a\do\b
	\do\c\do\d\do\e\do\f\do\g\do\h\do\i\do\j\do\k\do\l\do\m\do\n
	\do\o\do\p\do\q\do\r\do\s\do\t\do\u\do\v\do\w\do\x\do\y\do\z
	\do\.\do\@\do\\\do\/\do\!\do\_\do\|\do\;\do\>\do\]\do\)\do\,
	\do\?\do\'\do+\do\=\do\#}

% \usepackage{subfigure}
% \usepackage[justification=RaggedRight,labelfont=bf,font=small,textfont=normalfont,tableposition=below]{caption}

\setlength{\intextsep}{0.5em plus 0.2em minus  0.2em}
\setlength{\dbltextfloatsep}{0.5em plus 0.2em minus  0.2em}
\setlength{\dblfloatsep}{0.3em plus 0.2em minus  0.2em}
\setlength{\textfloatsep}{.3em}
\setlength{\floatsep}{.5em}
\setlength{\dbltextfloatsep}{.5em}
\setlength{\dblfloatsep}{.5em}
% \setlength{\subfigcapskip}{-.5em}
% \setlength{\subfigbottomskip}{0em}
% \setlength{\abovecaptionskip}{.3em}

% The following option reduces the space between words and letters. Can save 0.5-1 column
% from a 12-page paper, but makes the paper slightly less readable.
% \usepackage[subtle, lists=tight]{savetrees}

% \usepackage{enumitem}
% \setlist{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt}
% \setitemize{leftmargin=4mm}
% \setenumerate{leftmargin=4mm}



==> sections/exp-deepdive.tex <==
\subsection{\sys Deep Dive} \label{sec:exp:deepdive}
\subsubsection{Understand the dynamics}

==> sections/figures/cellular-tput.tex <==
\begin{figure}[t!]
	% \vspace{-0.1cm}
	\centering
	\includegraphics[width=0.7\columnwidth]{figures/cellular-tput.pdf}
	\vspace{-0.3cm}
	\caption{\sys can adapt to rapidly changing cellular network conditions.}
	\label{fig:exp:cellular-tput}
	\vspace{-0.4cm}
\end{figure}

==> sections/figures/conv-stability.tex <==
\begin{figure}[t!]
	\vspace{-0.1cm}
	\centering
	\includegraphics[width=0.6\columnwidth]{figures/converge.pdf}
	\vspace{-0.4cm}
	\caption{Convergence Time vs Stability}
	\label{fig:exp:fairness:conv}
	\vspace{-0.5cm}
\end{figure}

==> sections/figures/friend.tex <==
\begin{figure}[t]
    \centering
	\includegraphics[width=0.7\columnwidth]{figures/friendliness.pdf}
	\vspace{-0.3cm}
	\caption{Throughput ratio to CUBIC of various CC schemes. A ratio of 1 indicates optimal friendliness.}
	\label{fig:exp:friendliness}
	\vspace{-0.5cm}
\end{figure}

==> sections/figures/infer.tex <==
\begin{figure}[t]
	\vspace{-0.25cm}
	\centering
	\includegraphics[width=0.7\columnwidth]{figures/infer}
	\vspace{-0.2cm}
	\caption{\sys Inference Framework}
	\label{fig:inference}
	\vspace{-0.5cm}
\end{figure}

==> sections/figures/motiv.tex <==
\begin{figure*}[ht!]
    \vspace{-0.1cm}
    \centering
    \begin{minipage}[t]{0.48\textwidth}
    \vspace{0pt}
    \subfigure[Aurora is very unfair.]{\label{fig:motiv:aurora-unfair}\includegraphics[width=0.49\columnwidth]{figures/aurora-unfair.pdf}}
    \subfigure[Vivace converges slowly.]{\label{fig:motiv:vivace:slow}\includegraphics[width=0.49\columnwidth]{figures/vivace-slow-resp.pdf}}
    \vspace{-0.5cm}
    \caption{Existing learning-based algorithms fail to fast converge to fairness with stability.}
    \end{minipage}%
    \hfill 
    \begin{minipage}[t]{0.48\textwidth}
    \vspace{-0.5pt}
    \subfigure[Vivace \emph{could} converge quickly.]{\includegraphics[width=0.49\columnwidth]{figures/vivace-tuned.pdf}\label{fig:motiv:vivace:tune}}
    \subfigure[Vivace introduces instability.]{\includegraphics[width=0.49\columnwidth]{figures/vivace-tuned-bad-original.pdf}\label{fig:motiv:vivace:instability}}
    \vspace{-0.5cm}
    \caption{Enhanced Vivace performs diversely.}
    \vspace{-0.8cm}
    \end{minipage}
    \vspace{-0.5cm}
\end{figure*}

==> sections/marl-train.tex <==
\section{Training Algorithm of \sys}\label{sec:design:train:algo}


==> sections/overview.tex <==
\section{Overview}
In this section, we overview the framework of \sys and demonstrate the design challenges of \sys. 





